Estimating Endogenous Coalitional Mergers: Merger Costs and Assortativeness of Size and Specialization

I present a structural empirical model of a one-sided one-to-many matching with complementarities to quantify the effect of subsidy design on endogenous merger matching. I investigate shipping mergers and consolidations in Japan in 1964. At the time, 95 firms formed six large groups. I find that the existence of unmatched firms enables us to recover merger costs, and the importance of technological diversification varies across carrier and firm types. The counterfactual simulations show that 20 \% of government subsidy expenditures could have been cut. The government could have possibly changed the equilibrium number of groups to between one and six.

==> 09_4_results.tex <==
\section{Results}\label{sec:results}



\subsection{Investigation of the shape of the objective function on a few observed characteristics}\label{subsec:estimation_a_few_variables}\hspace*{\fill} \\

It is known that the maximum score estimator may not be good at handling high-dimensional observed covariates because many possible combinations of parameters are evaluated as true parameters within the discontinuous objective function. Before proceeding with a full model with many observed characteristics, in Section \ref{subsec:estimation_a_few_variables}, I investigate the shape of the objective function with a single characteristic as in \cite{bajari2008evaluating}. 

\begin{figure}[htbp]
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_score_only_x1_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_score_only_x2_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_score_only_x3_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_score_only_x4_shared_subsidy.png}
  \end{center}
 \end{minipage}\\
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_score_only_x5_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_score_only_x6_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_score_only_x7_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_score_only_x8_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \caption{Maximum rank objective function across a single different parameter. I include $\beta_0=+1$ for all specifications.}
 \label{fg:plot_score_betas_single_X_only}
\end{figure}

\begin{figure}[htbp]
 \begin{minipage}{0.45\hsize}
  \begin{center}
   \includegraphics[width=70mm]{figuretable/plot_score_only_gamma_shared_subsidy.png}
  \end{center}
 \end{minipage}
  \begin{minipage}{0.45\hsize}
  \begin{center}
   \includegraphics[width=70mm]{figuretable/plot_score_only_gamma_to_buyer_subsidy.png}
  \end{center}
 \end{minipage}
 \caption{\textbf{Maximum rank objective function across different parameters $\beta$ and merger cost $\gamma$ under different calibrated subsidy sensitivity $\delta$}. I include $\beta_0=+1$ for all specifications.}
 \label{fg:plot_score_delta_single_X_only}
\end{figure}

Figure \ref{fg:plot_score_betas_single_X_only} reports the shapes of the maximum score objective function \eqref{eq:score_function_detail} given the data when I include only one observed characteristic about post-merger size effects and technological specialization and fix subsidy sensitivity $\delta$ and merger cost $\gamma$ to zeros while fixing the normalized coefficient of the interaction term of total tonnage size to one, i.e., $\beta_0=+1$. First, the upper panels show results about economies of scale. I find that for $\beta_1,\beta_2$ and $\beta_3$, the objective function attains its maximum between 100 and 300, which implies that the ranges are too large to provide informative bounds. Also, the identified sets of $\beta_1$ and $\beta_3$ seem unbounded. On the other hand, for $\beta_4$, the objective function attains its maximum between 5 and 10 which is a relatively tight bound. Second, the lower panels show results about economies of scope. I find that almost all parameters can be point-identified but the objective function for $\beta_6$ is not single-peaked within a small domain, which suggests that set estimation with a 95 \% confidence interval would be more reliable than point-estimation. Figure \ref{fg:plot_score_delta_single_X_only} reports the shape of the maximum score objective function \eqref{eq:score_function_detail} under different calibrated subsidy sensitivity $\delta$. I find that merger cost $\gamma$ can be point-identified under both subsidy specifications but the maximum of the objective function is robust to the choice of the calibrated parameter only under the second subsidy specification.

Figure \ref{fg:plot_score_betas_two_X} adds varying merger cost $\gamma$ to the previous single-variable maximum score objective function. The bright yellow areas are the set of global maximizers. Although the sets of maximizers for $\beta_6$ and $\beta_8$ are difficult to show the boundedness graphically, I confirm that all sets of global maximizers are bounded so that I can construct 95 \% confidence intervals. However, I notice that the discontinuous objective function has multiple local optima at discrete points which may induce incorrect estimation. This is natural in real data. To alleviate the problem, I implement 10,000 population seeds (100 population seeds from 100 starting values) in DE algorithm for point estimation. 

To conclude, through the diagnoses of the shape of the objective function given the data, first, I find that some parameters for economies of scale such as $\beta_1$ and $\beta_3$ do not provide tight bounds in univariate estimation. I interpret that the total tonnage size whose coefficient is normalized to $+1$ explains not only the most parts of economies of scale in each carrier type but also the most parts of merger incentive to predict pairwise inequalities. This is because the number of achieved correct pairwise inequalities are approximately the same across all specifications. This also implies that about 3.7 percent of inequalities are unreasonable for all specifications. Second, almost all parameters provide relatively tight bounds in the estimation with at most two variables. This implies that the total tonnage size does not fully explain the balanced contribution of the post-merger size effects and technological specialization, and merger cost to pairwise inequalities.



\begin{figure}[htbp]
\begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_contour_score_two_variables_merger_cost_x1_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_contour_score_two_variables_merger_cost_x2_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_contour_score_two_variables_merger_cost_x3_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_contour_score_two_variables_merger_cost_x4_shared_subsidy.png}
  \end{center}
 \end{minipage}\\
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_contour_score_two_variables_merger_cost_x5_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_contour_score_two_variables_merger_cost_x6_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_contour_score_two_variables_merger_cost_x7_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.24\hsize}
  \begin{center}
   \includegraphics[width=40mm]{figuretable/plot_contour_score_two_variables_merger_cost_x8_shared_subsidy.png}
  \end{center}
 \end{minipage}
 \caption{\textbf{Maximum rank objective function across a single different parameter}. I include $\beta_0=+1$, $\delta=5$, and merger cost $\gamma$ (Y-axis) for all specifications. In the lower second and fourth panels, it is difficult to illustrate these bounded sets of maximizers because these bound regions face sudden decrease of the objective value which suppresses other colored domains. The boundedness of these two cases is confirmed numerically.}
 \label{fg:plot_score_betas_two_X}
\end{figure}

\subsection{Estimation results on two observed characteristics}\label{subsec:estimation_two_variables}\hspace*{\fill} \\

Continuing the steps in Section \ref{subsec:estimation_a_few_variables}, Table \ref{tb:score_results_two_variables} reports the estimation results with two observed characteristics and merger cost. The numbers in parentheses are 95 \% confidence intervals via subsampling. Estimation details are summarized in the footnote of Table \ref{tb:score_results_two_variables}. I normalized $\beta_0$ to $+1$ for identification. I estimate the other parameters separately under the normalization and pick the vector with the highest number of satisfied inequalities. The number of inequalities for the full sample is $17,870$. Almost all estimated parameters are within the sets of maximizers confirmed graphically in Figure \ref{fg:plot_score_betas_two_X}. As found in Section \ref{subsec:identification_monte_carlo}, the identification of the upper bound of $\delta$ is difficult. To deal with the problem, I find in the preliminary point estimation that $\delta=5$ achieves the maximum score as the integer lower bound of $\delta$ so that I calibrate $\delta=5$ for all specifications. The robustness checks are in Appendix \ref{sec:robustness_check}. Thus, I assume the worst case regarding $\delta$.

I begin discussing the estimated signs in Table \ref{tb:score_results_two_variables}. First, all specifications report the robust result that the estimated coefficient of merger cost $\gamma$ is positive, which means that a merger incurs significant costs. Second, in columns 1 to 4, I find that the point-estimated coefficients of economies of scale for $\beta_1$, $\beta_2$, and $\beta_3$ are positive but negative for $\beta_4$. Also, the 95 \% confidence intervals for $\beta_2$ and $\beta_4$ cover zero which implies that the signs are ambiguous. This implies that economies of scale exist but these are ambiguous for some carrier types. In columns 5 to 8, I find that the point-estimated coefficients of economies of scope are negative for $\beta_5,\beta_7$  but positive for $\beta_6$ and $\beta_8$. This means that technological diversification on carrier types such as linear, special contributes to merger incentive, on the other hand, technological specialization on tramper and tanker is important for merger incentive. However, the 95 \% confidence interval shows that the estimated sign of $\beta_8$ is ambiguous.

Table \ref{tb:ratio_score_results_two_variables} reports the relative importance of each variable compared with merger cost in the first row. For a matching maximum score estimator, the relative sizes of coefficients are important. The second row shows the comparable level of estimated coefficients between the observed characteristics. For example, I interpret that the economies of scale in tramper shipping ($\beta_3/|\gamma|=6.0$) is 1.5 times more important for merger incentive than the economies of scope in liner shipping ($\beta_1/|\gamma|=4.0$). On the other hand, the economies of scope in liner shipping ($\beta_5/|\gamma|=-5.0$) is five times more important for merger incentive than the economies of scope in special ($\beta_7/|\gamma|=-1.0$). In conclusion, I find that both post-merger size effects and technological specialization are important for merger incentive, however, the importance levels and signs significantly vary in each carrier type. 

\begin{landscape}
{
\begin{table}[!htbp] \centering 
  \caption{\textbf{Results of matching maximum rank estimator with two observed variables}} 
  \label{tb:score_results_two_variables} 
  {\fontsize{2.0}{3.0}\selectfont
  \input{figuretable/score_results_two_variables_shared_subsidy}
\begin{tablenotes}
\textit{Note:} The objective function was numerically maximized using differential evolution (DE) algorithm in \texttt{BlackBoxOptim.jl} package. For DE algorithm, I require setting the domain of parameters and the number of population seeds so that I fix the former to $[-1000, 2000]$ for $\omega$ and $[-200,200]$ for other parameters, and the latter to 100. For point estimation, 100 runs were performed for all specifications. The reported point estimates are the best-found maxima. The parentheses are 95 \% confidence intervals which are computed by taking the 2.5th percentile
and the 97.5th percentile of the empirical sampling distribution of estimated parameters. Subsampling uses 200 replications and 42 firms (all 12 main firms and 30 non-main firms out of 106) per replication (sampled without replacement). Subsampled confidence regions are not necessarily symmetric around the point estimate. For each subsample, we evaluate the valuation functions using the full samples, whether all of the firms are among the subset of 118 or not. Parameters that can take on only a finite number of values (here +1) converge at an arbitrarily fast rate, they are superconsistent (denoted by (S)). The unit of measure of economies of scale is a million of DW tonnage. The sub-indices $b$ and $t$ mean the buyer's and target coalition's covariates. Subsampled confidence regions are not necessarily symmetric around the point estimate.
   \end{tablenotes}
   }
\end{table} 

{
\begin{table}[!htbp] \centering 
  \caption{\textbf{Relative levels of matching maximum rank estimator in Table \ref{tb:score_results_two_variables}}} 
  \label{tb:ratio_score_results_two_variables} 
  {\fontsize{2.0}{3.0}\selectfont
  \input{figuretable/ratio_score_results_two_variables_shared_subsidy}
   }
\end{table} 
}

}
\end{landscape}



\subsection{Estimation results on two observed characteristics for 12 main firms}\label{subsec:estimation_two_variables_main_firms_only}\hspace*{\fill} \\

Finally, I report the maximum rank results on two observed characteristics by focusing only on 12 main firms each of which can be either a buyer, a seller, or staying unmatched. Although the one-to-many matching market I investigate in this article is rare, the estimation procedure is not only applicable to market(s) where large firms compete even in a single market but also implementable for counterfactual analyses in a tractable size market as shown in Section \ref{sec:counter_factual}.  I find the lower bound of $\delta$ in the preliminary point estimation and fix $\delta$ to the value as a calibrated parameter ($\delta=1000$).\footnote{The value is much larger than the previous value in Table \ref{tb:score_results_two_variables}. This is because the subsample includes only matched groups which consist of much fewer firms and interaction terms of explanatory variables are smaller than the full sample. Thus, to explain the difference between pre-subsidy and post-subsidy matching outcomes, the subsidy term will have a more important role. The robustness checks are in Appendix \ref{sec:robustness_check}.} The goodness of fit in Table \ref{tb:score_results_two_variables_main_firms_only} is similar to the results in Table \ref{tb:score_results_two_variables}.

Table \ref{tb:score_results_two_variables_main_firms_only} reports the maximum rank results for the subsample. Since I use 12 main firms in this section, I could not construct 95 \% confidence intervals with enough subsampled data. Instead, the numbers of bracket mean lower and upper bounds of a set of maximizers of the maximum rank estimator. I find that estimated signs of many parameters are consistent with Table \ref{tb:score_results_two_variables}. However, some parameters such as $\beta_4$, $\beta_5$, and $\beta_8$ show different signs. These discrepancies might come from the ambiguity of signs in Table \ref{tb:score_results_two_variables} and differences of carrier type composition between 12 main firms and dropped other firms. In Section \ref{sec:counter_factual}, I simulate counterfactual analyses for 12 main firms based on estimated parameters in Table \ref{tb:score_results_two_variables_main_firms_only} to answer several policy questions about subsidy effects on merger configurations and matching outcomes.

{
\begin{table}[!htbp] \centering 
  \caption{\textbf{Results of matching maximum rank estimator with two observed variables for 12 main firms.} The numbers of bracket are lower and upper bounds of a set of maximizers of the maximum rank estimator.} 
  \label{tb:score_results_two_variables_main_firms_only} 
  {\fontsize{2.0}{3.0}\selectfont
  \input{figuretable/score_results_two_variables_shared_subsidy_main_firms_only}
  }
\end{table} 
}







==> figuretable/counterfactual_subsidy_amount.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcccc}
\toprule 
 &  & Point Estimate Scenario & The most expensive scenario & The cheapest expenditure scenario \\
merger cost $\gamma$ &  & $\gamma=-0.69$ & $\gamma=-6.2$ & $\gamma=-0.46$ \\
 &  & Avg $\sharp$ of groups ($\sharp$ of unmatched) & Avg $\sharp$ of groups ($\sharp$ of unmatched) & Avg $\sharp$ of groups ($\sharp$ of unmatched) \\
\midrule 
subsidy amount ($M$) &  &  &  &  \\
 &  &  &  &  \\
100 (0.1) &  & 3.0 (6.0) & 4.0 (2.0) & 3.0 (6.0) \\
 &  &  &  &  \\
1000 (1.0) (benchmark, data) &  & 2.0 (7.0) & 3.0 (6.0) & 2.0 (7.0) \\
 &  &  &  &  \\
5000 (5.0) &  & 2.0 (7.0) & 4.0 (4.0) & 1.0 (8.0) \\
 &  &  &  &  \\
10000 (10.0) &  & 2.0 (7.0) & 2.0 (7.0) & 2.0 (7.0) \\
 &  &  &  &  \\
30000 (30.0) &  & 2.0 (7.0) & 2.0 (7.0) & 2.0 (7.0) \\
 &  &  &  &  \\
50000 (50.0)) &  & 2.0 (7.0) & 1.0 (8.0) & 1.0 (7.0) \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/counterfactual_subsidy_threshold.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcccc}
\toprule 
 &  & Point Estimate Scenario & The most expensive scenario & The cheapest expenditure scenario \\
merger cost $\gamma$ &  & $\gamma=-0.69$ & $\gamma=-6.2$ & $\gamma=-0.46$ \\
 &  & Avg $\sharp$ of groups ($\sharp$ of unmatched) & Avg $\sharp$ of groups ($\sharp$ of unmatched) & Avg $\sharp$ of groups ($\sharp$ of unmatched) \\
\midrule 
subsidy threshold (DW) &  &  &  &  \\
 &  &  &  &  \\
1 million ton (benchmark, data) &  & 2.0 (7.0) & 3.0 (6.0) & 2.0 (7.0) \\
 &  &  &  &  \\
2 million ton &  & 4.0 (2.0) & 4.0 (3.0) & 4.0 (2.0) \\
 &  &  &  &  \\
3 million ton &  & 4.0 (1.0) & 4.0 (2.0) & 3.0 (1.0) \\
 &  &  &  &  \\
4 million ton &  & 4.0 (1.0) & 4.0 (2.0) & 4.0 (1.0) \\
 &  &  &  &  \\
5 million ton &  & 4.0 (2.0) & 4.0 (2.0) & 3.0 (1.0) \\
 &  &  &  &  \\
6 million ton &  & 4.0 (2.0) & 4.0 (2.0) & 4.0 (2.0) \\
 &  &  &  &  \\
7 million ton &  & 4.0 (2.0) & 4.0 (2.0) & 4.0 (2.0) \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta_with_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc|lccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  & $\beta_2$ &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 0.12 & 0.13 & 0.12 & 0.05 & 0.02 &  & 3.8 & 4.61 & 4.81 & 4.94 & 4.38 \\
 &  & RMSE & (0.9) & (0.47) & (0.44) & (0.28) & (0.16) &  & (4.82) & (5.41) & (5.56) & (5.71) & (5.25) \\
 & T & Bias & 0.12 & 0.13 & 0.12 & 0.05 & 0.01 &  & 3.78 & 4.61 & 4.77 & 5.03 & 4.32 \\
 &  & RMSE & (0.9) & (0.47) & (0.44) & (0.28) & (0.17) &  & (4.79) & (5.41) & (5.55) & (5.79) & (5.19) \\
 & U & Bias & 0.15 & 0.14 & 0.11 & 0.05 & 0.01 &  & 3.84 & 4.55 & 4.86 & 5.08 & 4.31 \\
 &  & RMSE & (0.96) & (0.48) & (0.44) & (0.28) & (0.17) &  & (4.82) & (5.37) & (5.62) & (5.82) & (5.19) \\
 & Non & Bias & 0.12 & 0.14 & 0.11 & 0.05 & 0.01 &  & 3.82 & 4.55 & 4.86 & 5.08 & 4.31 \\
 &  & RMSE & (0.9) & (0.48) & (0.44) & (0.28) & (0.17) &  & (4.79) & (5.37) & (5.62) & (5.82) & (5.19) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.03 & 0.0 & 0.0 & 0.0 & 0.02 & 0.0 & 0.03 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.16 & 0.08 & 0.14 & 0.05 & 0.02 &  & 5.03 & 5.69 & 5.66 & 5.89 & 5.56 \\
 &  & RMSE & (0.65) & (0.28) & (0.47) & (0.28) & (0.16) &  & (5.88) & (6.31) & (6.3) & (6.55) & (6.29) \\
 & T & Bias & 0.11 & 0.08 & 0.14 & 0.05 & 0.02 &  & 5.06 & 5.69 & 5.62 & 5.86 & 5.54 \\
 &  & RMSE & (0.45) & (0.28) & (0.47) & (0.28) & (0.16) &  & (5.89) & (6.31) & (6.28) & (6.52) & (6.27) \\
 & U & Bias & 0.15 & 0.08 & 0.14 & 0.05 & 0.01 &  & 5.13 & 5.63 & 5.62 & 5.9 & 5.57 \\
 &  & RMSE & (0.57) & (0.29) & (0.47) & (0.28) & (0.16) &  & (5.93) & (6.26) & (6.28) & (6.56) & (6.29) \\
 & Non & Bias & 0.11 & 0.08 & 0.14 & 0.05 & 0.01 &  & 5.11 & 5.63 & 5.71 & 5.9 & 5.57 \\
 &  & RMSE & (0.45) & (0.29) & (0.47) & (0.28) & (0.16) &  & (5.91) & (6.26) & (6.36) & (6.56) & (6.29) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 1.67 & 2.86 & 3.85 & 5.55 & 10.95 & -1.0 & 1.67 & 2.86 & 3.85 & 5.55 & 10.95 \\
 & U,T & Bias & 0.59 & 0.44 & 0.25 & 0.19 & 0.16 &  & 2.65 & 2.3 & 2.39 & 2.54 & 2.56 \\
 &  & RMSE & (1.62) & (1.2) & (0.56) & (0.47) & (0.31) &  & (4.52) & (4.14) & (4.2) & (4.37) & (4.17) \\
 & T & Bias & 0.66 & 0.35 & 0.19 & 0.16 & 0.12 &  & 2.96 & 2.65 & 3.45 & 3.9 & 3.21 \\
 &  & RMSE & (1.75) & (1.1) & (0.48) & (0.42) & (0.28) &  & (4.71) & (4.17) & (5.05) & (5.51) & (4.64) \\
 & U & Bias & 0.59 & 0.46 & 0.25 & 0.2 & 0.17 &  & 2.63 & 2.25 & 2.26 & 2.43 & 2.38 \\
 &  & RMSE & (1.63) & (1.22) & (0.56) & (0.47) & (0.32) &  & (4.49) & (4.12) & (4.03) & (4.23) & (3.93) \\
 & Non & Bias & 0.66 & 0.34 & 0.18 & 0.17 & 0.12 &  & 2.94 & 2.95 & 3.41 & 3.75 & 3.11 \\
 &  & RMSE & (1.75) & (1.1) & (0.48) & (0.43) & (0.28) &  & (4.71) & (4.5) & (5.02) & (5.38) & (4.52) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 5.67 & 11.02 & 16.18 & 26.42 & 51.09 & -2.0 & 5.67 & 11.02 & 16.18 & 26.42 & 51.09 \\
 & U,T & Bias & 0.58 & 0.46 & 0.45 & 0.41 & 0.44 &  & -0.37 & -0.08 & 0.04 & 0.06 & -0.03 \\
 &  & RMSE & (1.04) & (0.74) & (0.75) & (0.62) & (0.65) &  & (1.23) & (0.64) & (0.6) & (0.49) & (0.46) \\
 & T & Bias & 0.5 & 0.71 & 0.11 & 0.22 & 0.13 &  & 2.14 & 4.19 & 5.17 & 5.67 & 5.81 \\
 &  & RMSE & (1.45) & (2.08) & (0.37) & (0.64) & (0.38) &  & (4.29) & (6.15) & (6.57) & (6.97) & (6.97) \\
 & U & Bias & 0.59 & 0.47 & 0.45 & 0.41 & 0.44 &  & -0.38 & -0.08 & 0.04 & 0.08 & -0.01 \\
 &  & RMSE & (1.04) & (0.75) & (0.75) & (0.6) & (0.65) &  & (1.23) & (0.64) & (0.59) & (0.45) & (0.45) \\
 & Non & Bias & 0.61 & 0.71 & 0.16 & 0.22 & 0.13 &  & 2.09 & 4.26 & 5.17 & 5.7 & 5.77 \\
 &  & RMSE & (1.74) & (2.08) & (0.62) & (0.64) & (0.38) &  & (4.23) & (6.21) & (6.56) & (7.0) & (6.92) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 8.92 & 17.46 & 25.82 & 42.48 & 84.4 & -3.0 & 8.92 & 17.46 & 25.82 & 42.48 & 84.4 \\
 & U,T & Bias & -0.32 & 0.49 & 0.37 & 0.27 & 0.23 &  & -1.3 & -0.75 & -0.36 & -0.05 & 0.02 \\
 &  & RMSE & (2.3) & (0.99) & (0.65) & (0.49) & (0.43) &  & (2.5) & (1.79) & (1.05) & (0.69) & (0.58) \\
 & T & Bias & 1.34 & 0.96 & 0.45 & 0.12 & 0.44 &  & 1.57 & 5.28 & 5.53 & 6.21 & 6.61 \\
 &  & RMSE & (3.98) & (3.13) & (1.99) & (0.99) & (1.69) &  & (5.37) & (7.29) & (7.07) & (7.16) & (7.81) \\
 & U & Bias & -0.32 & 0.48 & 0.35 & 0.26 & 0.21 &  & -1.3 & -0.73 & -0.32 & -0.03 & 0.05 \\
 &  & RMSE & (2.3) & (1.01) & (0.64) & (0.49) & (0.39) &  & (2.5) & (1.81) & (1.0) & (0.69) & (0.54) \\
 & Non & Bias & 1.32 & 1.04 & 0.45 & 0.12 & 0.46 &  & 1.72 & 5.39 & 5.51 & 6.19 & 6.57 \\
 &  & RMSE & (3.91) & (3.27) & (1.99) & (0.99) & (1.7) &  & (5.39) & (7.36) & (7.06) & (7.14) & (7.78) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta_with_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc|lccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  & $\beta_2$ &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 0.46 & 0.14 & 0.14 & 0.04 & 0.01 &  & -0.24 & -0.3 & -0.72 & -1.82 & -1.63 \\
 &  & RMSE & (1.88) & (0.48) & (0.47) & (0.29) & (0.16) &  & (5.39) & (5.66) & (5.74) & (5.91) & (5.91) \\
 & T & Bias & 0.56 & 0.11 & 0.14 & 0.04 & 0.0 &  & -0.24 & -0.22 & -0.76 & -1.71 & -1.64 \\
 &  & RMSE & (1.99) & (0.39) & (0.47) & (0.29) & (0.16) &  & (5.28) & (5.58) & (5.78) & (5.85) & (5.96) \\
 & U & Bias & 0.53 & 0.11 & 0.14 & 0.04 & 0.0 &  & -0.27 & -0.28 & -0.74 & -1.7 & -1.58 \\
 &  & RMSE & (1.96) & (0.39) & (0.47) & (0.29) & (0.16) &  & (5.25) & (5.53) & (5.75) & (5.86) & (5.98) \\
 & Non & Bias & 0.56 & 0.11 & 0.14 & 0.04 & 0.0 &  & -0.27 & -0.31 & -0.74 & -1.7 & -1.58 \\
 &  & RMSE & (1.99) & (0.39) & (0.47) & (0.29) & (0.16) &  & (5.25) & (5.56) & (5.75) & (5.86) & (5.98) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.02 & 0.0 & 0.0 & 0.0 & 0.02 & 0.0 & 0.02 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.39 & 0.18 & 0.14 & 0.04 & 0.01 &  & 0.45 & 0.28 & 0.28 & -0.82 & -0.94 \\
 &  & RMSE & (1.74) & (0.67) & (0.47) & (0.29) & (0.16) &  & (5.55) & (5.41) & (5.7) & (5.69) & (5.8) \\
 & T & Bias & 0.48 & 0.17 & 0.14 & 0.04 & 0.0 &  & 0.41 & 0.25 & 0.34 & -0.82 & -0.78 \\
 &  & RMSE & (1.86) & (0.66) & (0.47) & (0.29) & (0.16) &  & (5.4) & (5.45) & (5.72) & (5.69) & (5.81) \\
 & U & Bias & 0.44 & 0.18 & 0.14 & 0.04 & 0.0 &  & 0.38 & 0.2 & 0.26 & -0.7 & -0.56 \\
 &  & RMSE & (1.83) & (0.66) & (0.47) & (0.29) & (0.16) &  & (5.37) & (5.38) & (5.71) & (5.65) & (5.81) \\
 & Non & Bias & 0.48 & 0.18 & 0.14 & 0.04 & 0.0 &  & 0.38 & 0.17 & 0.26 & -0.7 & -0.56 \\
 &  & RMSE & (1.86) & (0.66) & (0.47) & (0.29) & (0.16) &  & (5.37) & (5.41) & (5.71) & (5.65) & (5.81) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 1.56 & 2.81 & 3.92 & 5.84 & 10.93 & -1.0 & 1.56 & 2.81 & 3.92 & 5.84 & 10.93 \\
 & U,T & Bias & 0.38 & 0.32 & 0.13 & 0.03 & 0.02 &  & -3.76 & -5.0 & -4.88 & -4.35 & -4.75 \\
 &  & RMSE & (1.72) & (1.07) & (0.43) & (0.21) & (0.15) &  & (5.38) & (5.64) & (5.63) & (5.13) & (5.55) \\
 & T & Bias & 0.42 & 0.28 & 0.16 & 0.04 & 0.02 &  & -3.02 & -3.11 & -2.99 & -2.52 & -2.89 \\
 &  & RMSE & (1.48) & (1.05) & (0.48) & (0.25) & (0.15) &  & (5.4) & (5.89) & (5.47) & (5.33) & (5.32) \\
 & U & Bias & 0.37 & 0.3 & 0.12 & 0.04 & 0.01 &  & -3.86 & -5.04 & -5.08 & -4.52 & -4.98 \\
 &  & RMSE & (1.72) & (1.06) & (0.44) & (0.22) & (0.15) &  & (5.41) & (5.66) & (5.77) & (5.23) & (5.68) \\
 & Non & Bias & 0.4 & 0.28 & 0.15 & 0.04 & 0.02 &  & -3.02 & -2.97 & -2.88 & -2.51 & -2.91 \\
 &  & RMSE & (1.47) & (1.05) & (0.48) & (0.25) & (0.15) &  & (5.39) & (5.91) & (5.58) & (5.31) & (5.34) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 5.52 & 10.93 & 16.08 & 26.29 & 51.02 & -2.0 & 5.52 & 10.93 & 16.08 & 26.29 & 51.02 \\
 & U,T & Bias & 0.28 & 0.07 & 0.04 & 0.04 & 0.02 &  & -4.42 & -4.63 & -4.51 & -4.43 & -4.35 \\
 &  & RMSE & (0.88) & (0.31) & (0.22) & (0.16) & (0.11) &  & (4.98) & (5.12) & (5.06) & (5.07) & (4.9) \\
 & T & Bias & 0.13 & 0.4 & 0.52 & 0.38 & 0.07 &  & -1.13 & -0.25 & 0.12 & 0.81 & 0.81 \\
 &  & RMSE & (1.4) & (1.97) & (1.79) & (0.96) & (0.28) &  & (5.47) & (5.23) & (5.93) & (5.78) & (5.36) \\
 & U & Bias & 0.28 & 0.05 & 0.03 & 0.03 & 0.02 &  & -4.46 & -4.69 & -4.63 & -4.61 & -4.52 \\
 &  & RMSE & (0.88) & (0.29) & (0.2) & (0.15) & (0.1) &  & (5.0) & (5.13) & (5.12) & (5.16) & (4.99) \\
 & Non & Bias & 0.23 & 0.41 & 0.53 & 0.38 & 0.07 &  & -1.02 & -0.3 & -0.13 & 0.72 & 0.8 \\
 &  & RMSE & (1.57) & (1.97) & (1.79) & (0.96) & (0.28) &  & (5.3) & (5.26) & (5.87) & (5.75) & (5.37) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 8.87 & 17.34 & 25.78 & 42.5 & 84.45 & -3.0 & 8.87 & 17.34 & 25.78 & 42.5 & 84.45 \\
 & U,T & Bias & -0.49 & 0.1 & 0.08 & 0.0 & 0.03 &  & -2.67 & -3.88 & -3.31 & -3.78 & -3.64 \\
 &  & RMSE & (2.49) & (0.54) & (0.39) & (0.19) & (0.15) &  & (4.18) & (4.38) & (3.91) & (4.32) & (4.12) \\
 & T & Bias & -0.12 & 0.11 & 0.24 & 0.32 & 0.04 &  & 0.78 & 2.51 & 1.93 & 3.53 & 2.8 \\
 &  & RMSE & (4.31) & (3.25) & (2.46) & (1.63) & (0.19) &  & (5.93) & (6.71) & (6.03) & (6.49) & (6.63) \\
 & U & Bias & -0.5 & 0.09 & 0.06 & 0.0 & 0.01 &  & -2.7 & -4.08 & -3.5 & -3.98 & -3.86 \\
 &  & RMSE & (2.48) & (0.54) & (0.36) & (0.18) & (0.11) &  & (4.21) & (4.52) & (4.01) & (4.42) & (4.27) \\
 & Non & Bias & -0.1 & 0.11 & 0.23 & 0.34 & 0.06 &  & 0.9 & 2.51 & 1.83 & 3.42 & 2.94 \\
 &  & RMSE & (4.32) & (3.25) & (2.47) & (1.62) & (0.27) &  & (5.96) & (6.71) & (5.91) & (6.49) & (6.64) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta_without_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc|lccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  & $\beta_2$ &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 1.11 & 0.29 & 0.26 & 0.25 & 0.18 &  & 1.27 & 0.5 & 0.7 & 0.49 & 0.33 \\
 &  & RMSE & (2.36) & (0.71) & (0.7) & (0.46) & (0.36) &  & (2.5) & (1.24) & (1.36) & (0.89) & (0.65) \\
 & T & Bias & 1.16 & 0.26 & 0.25 & 0.25 & 0.18 &  & 1.25 & 0.44 & 0.7 & 0.52 & 0.35 \\
 &  & RMSE & (2.43) & (0.67) & (0.7) & (0.46) & (0.36) &  & (2.5) & (1.19) & (1.36) & (0.9) & (0.67) \\
 & U & Bias & 1.1 & 0.29 & 0.25 & 0.26 & 0.17 &  & 1.28 & 0.5 & 0.7 & 0.5 & 0.34 \\
 &  & RMSE & (2.36) & (0.7) & (0.7) & (0.47) & (0.35) &  & (2.5) & (1.27) & (1.36) & (0.89) & (0.65) \\
 & Non & Bias & 1.21 & 0.27 & 0.25 & 0.26 & 0.18 &  & 1.26 & 0.49 & 0.71 & 0.51 & 0.36 \\
 &  & RMSE & (2.46) & (0.69) & (0.7) & (0.47) & (0.36) &  & (2.51) & (1.27) & (1.36) & (0.9) & (0.68) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 & 0.0 & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.94 & 0.47 & 0.72 & 0.7 & 0.52 &  & 0.32 & 0.19 & 0.03 & 0.08 & 0.07 \\
 &  & RMSE & (2.18) & (0.92) & (1.03) & (0.92) & (0.73) &  & (1.19) & (0.52) & (0.29) & (0.21) & (0.18) \\
 & T & Bias & 0.89 & 0.48 & 0.74 & 0.7 & 0.54 &  & 0.32 & 0.18 & 0.03 & 0.08 & 0.07 \\
 &  & RMSE & (2.14) & (0.93) & (1.03) & (0.92) & (0.75) &  & (1.18) & (0.52) & (0.29) & (0.21) & (0.19) \\
 & U & Bias & 0.94 & 0.48 & 0.74 & 0.7 & 0.53 &  & 0.31 & 0.17 & 0.03 & 0.07 & 0.06 \\
 &  & RMSE & (2.18) & (0.93) & (1.03) & (0.92) & (0.75) &  & (1.19) & (0.52) & (0.29) & (0.21) & (0.18) \\
 & Non & Bias & 0.89 & 0.48 & 0.74 & 0.69 & 0.54 &  & 0.32 & 0.17 & 0.03 & 0.07 & 0.07 \\
 &  & RMSE & (2.14) & (0.93) & (1.03) & (0.92) & (0.75) &  & (1.18) & (0.52) & (0.29) & (0.21) & (0.19) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 1.7 & 3.22 & 4.31 & 6.68 & 12.6 & -1.0 & 1.7 & 3.22 & 4.31 & 6.68 & 12.6 \\
 & U,T & Bias & 1.27 & 0.96 & 0.78 & 0.71 & 0.7 &  & -0.43 & -0.14 & 0.03 & 0.1 & 0.13 \\
 &  & RMSE & (2.16) & (1.36) & (1.07) & (0.93) & (0.87) &  & (1.1) & (0.63) & (0.4) & (0.31) & (0.31) \\
 & T & Bias & 1.29 & 1.01 & 0.83 & 0.68 & 0.77 &  & -0.41 & -0.09 & 0.04 & 0.12 & 0.16 \\
 &  & RMSE & (2.24) & (1.59) & (1.11) & (0.86) & (0.94) &  & (1.14) & (0.6) & (0.36) & (0.29) & (0.34) \\
 & U & Bias & 1.37 & 0.96 & 0.77 & 0.75 & 0.73 &  & -0.46 & -0.15 & 0.03 & 0.08 & 0.13 \\
 &  & RMSE & (2.33) & (1.36) & (1.07) & (0.98) & (0.9) &  & (1.13) & (0.63) & (0.39) & (0.31) & (0.32) \\
 & Non & Bias & 1.29 & 1.01 & 0.84 & 0.7 & 0.79 &  & -0.42 & -0.09 & 0.03 & 0.12 & 0.16 \\
 &  & RMSE & (2.24) & (1.59) & (1.12) & (0.87) & (0.98) &  & (1.15) & (0.6) & (0.37) & (0.29) & (0.34) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 5.68 & 10.51 & 15.82 & 25.79 & 49.95 & -2.0 & 5.68 & 10.51 & 15.82 & 25.79 & 49.95 \\
 & U,T & Bias & 1.15 & 0.84 & 0.62 & 0.69 & 0.5 &  & -1.27 & -0.45 & -0.14 & -0.15 & 0.02 \\
 &  & RMSE & (2.35) & (1.18) & (0.83) & (0.92) & (0.69) &  & (2.5) & (1.05) & (0.61) & (0.57) & (0.58) \\
 & T & Bias & 1.35 & 1.36 & 0.56 & 0.59 & 0.61 &  & -0.74 & -0.47 & 0.03 & 0.2 & 0.36 \\
 &  & RMSE & (2.69) & (2.3) & (0.82) & (0.88) & (0.81) &  & (2.51) & (1.35) & (0.64) & (0.61) & (0.54) \\
 & U & Bias & 1.14 & 0.82 & 0.64 & 0.69 & 0.46 &  & -1.25 & -0.43 & -0.14 & -0.14 & 0.08 \\
 &  & RMSE & (2.34) & (1.16) & (0.85) & (0.91) & (0.61) &  & (2.51) & (1.03) & (0.61) & (0.57) & (0.45) \\
 & Non & Bias & 1.31 & 1.38 & 0.54 & 0.59 & 0.61 &  & -0.8 & -0.47 & 0.05 & 0.21 & 0.34 \\
 &  & RMSE & (2.66) & (2.31) & (0.8) & (0.88) & (0.79) &  & (2.42) & (1.35) & (0.63) & (0.61) & (0.55) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 7.69 & 14.85 & 22.13 & 36.13 & 72.04 & -3.0 & 7.69 & 14.85 & 22.13 & 36.13 & 72.04 \\
 & U,T & Bias & 0.48 & 0.57 & 0.47 & 0.46 & 0.52 &  & -1.6 & -0.57 & -0.26 & -0.07 & -0.15 \\
 &  & RMSE & (2.24) & (0.89) & (0.67) & (0.63) & (0.69) &  & (2.79) & (1.49) & (0.94) & (0.77) & (0.8) \\
 & T & Bias & 1.16 & 1.16 & 0.79 & 0.57 & 0.6 &  & 0.12 & 0.32 & -0.21 & 0.19 & 0.14 \\
 &  & RMSE & (3.08) & (2.15) & (1.43) & (0.9) & (0.81) &  & (4.0) & (2.95) & (1.84) & (1.0) & (0.72) \\
 & U & Bias & 0.46 & 0.57 & 0.5 & 0.46 & 0.5 &  & -1.56 & -0.57 & -0.3 & -0.05 & -0.11 \\
 &  & RMSE & (2.23) & (0.89) & (0.71) & (0.63) & (0.62) &  & (2.73) & (1.49) & (0.98) & (0.76) & (0.65) \\
 & Non & Bias & 1.37 & 1.26 & 0.8 & 0.57 & 0.6 &  & 0.21 & 0.24 & -0.2 & 0.19 & 0.14 \\
 &  & RMSE & (3.28) & (2.28) & (1.43) & (0.9) & (0.81) &  & (4.05) & (2.97) & (1.84) & (1.0) & (0.72) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta_without_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc|lccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  & $\beta_2$ &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 0.3 & 0.33 & 0.08 & 0.22 & 0.13 &  & 0.33 & 0.38 & 0.22 & 0.48 & 0.3 \\
 &  & RMSE & (1.23) & (0.91) & (0.29) & (0.44) & (0.27) &  & (1.17) & (1.04) & (0.65) & (0.85) & (0.63) \\
 & T & Bias & 0.27 & 0.32 & 0.09 & 0.23 & 0.14 &  & 0.35 & 0.37 & 0.22 & 0.49 & 0.32 \\
 &  & RMSE & (1.17) & (0.91) & (0.3) & (0.45) & (0.28) &  & (1.17) & (1.03) & (0.65) & (0.85) & (0.65) \\
 & U & Bias & 0.33 & 0.33 & 0.09 & 0.23 & 0.13 &  & 0.35 & 0.38 & 0.22 & 0.49 & 0.33 \\
 &  & RMSE & (1.3) & (0.91) & (0.3) & (0.45) & (0.28) &  & (1.17) & (1.04) & (0.65) & (0.85) & (0.65) \\
 & Non & Bias & 0.33 & 0.32 & 0.09 & 0.23 & 0.13 &  & 0.35 & 0.38 & 0.22 & 0.49 & 0.33 \\
 &  & RMSE & (1.3) & (0.91) & (0.3) & (0.45) & (0.28) &  & (1.17) & (1.04) & (0.65) & (0.85) & (0.65) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 & 0.0 & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.38 & 0.24 & 0.44 & 0.34 & 0.38 &  & -0.11 & 0.01 & -0.01 & 0.02 & -0.01 \\
 &  & RMSE & (1.32) & (0.5) & (0.84) & (0.59) & (0.54) &  & (1.61) & (0.44) & (0.29) & (0.21) & (0.17) \\
 & T & Bias & 0.49 & 0.23 & 0.44 & 0.35 & 0.38 &  & -0.13 & 0.01 & -0.02 & 0.01 & -0.0 \\
 &  & RMSE & (1.3) & (0.5) & (0.84) & (0.6) & (0.55) &  & (1.52) & (0.43) & (0.29) & (0.21) & (0.17) \\
 & U & Bias & 0.56 & 0.24 & 0.44 & 0.36 & 0.39 &  & -0.13 & 0.0 & -0.02 & 0.01 & -0.01 \\
 &  & RMSE & (1.41) & (0.5) & (0.84) & (0.61) & (0.55) &  & (1.57) & (0.43) & (0.29) & (0.21) & (0.17) \\
 & Non & Bias & 0.57 & 0.23 & 0.44 & 0.36 & 0.39 &  & -0.11 & 0.01 & -0.02 & 0.01 & -0.01 \\
 &  & RMSE & (1.41) & (0.5) & (0.84) & (0.61) & (0.55) &  & (1.56) & (0.43) & (0.29) & (0.21) & (0.17) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 1.8 & 3.05 & 4.38 & 6.56 & 12.76 & -1.0 & 1.8 & 3.05 & 4.38 & 6.56 & 12.76 \\
 & U,T & Bias & 0.85 & 0.35 & 0.19 & 0.21 & 0.15 &  & -1.31 & -0.54 & -0.25 & -0.33 & -0.27 \\
 &  & RMSE & (1.76) & (0.67) & (0.42) & (0.38) & (0.31) &  & (2.05) & (0.84) & (0.49) & (0.58) & (0.44) \\
 & T & Bias & 0.71 & 0.26 & 0.14 & 0.22 & 0.14 &  & -1.23 & -0.43 & -0.28 & -0.3 & -0.25 \\
 &  & RMSE & (1.78) & (0.59) & (0.37) & (0.39) & (0.3) &  & (2.02) & (0.73) & (0.59) & (0.57) & (0.42) \\
 & U & Bias & 0.92 & 0.35 & 0.19 & 0.19 & 0.15 &  & -1.39 & -0.53 & -0.25 & -0.31 & -0.27 \\
 &  & RMSE & (1.87) & (0.67) & (0.44) & (0.37) & (0.3) &  & (2.2) & (0.84) & (0.5) & (0.56) & (0.45) \\
 & Non & Bias & 0.75 & 0.28 & 0.14 & 0.23 & 0.14 &  & -1.3 & -0.48 & -0.28 & -0.31 & -0.27 \\
 &  & RMSE & (1.81) & (0.61) & (0.37) & (0.39) & (0.3) &  & (2.07) & (0.81) & (0.59) & (0.59) & (0.44) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 5.62 & 10.72 & 15.67 & 25.43 & 50.11 & -2.0 & 5.62 & 10.72 & 15.67 & 25.43 & 50.11 \\
 & U,T & Bias & 0.34 & 0.15 & 0.1 & 0.13 & 0.1 &  & -1.36 & -0.62 & -0.48 & -0.36 & -0.26 \\
 &  & RMSE & (1.38) & (0.41) & (0.29) & (0.28) & (0.24) &  & (2.39) & (0.99) & (0.76) & (0.63) & (0.5) \\
 & T & Bias & 0.2 & 0.39 & 0.36 & 0.23 & 0.09 &  & -1.41 & -0.75 & -0.69 & -0.59 & -0.2 \\
 &  & RMSE & (2.25) & (1.33) & (1.15) & (0.55) & (0.24) &  & (2.58) & (1.73) & (1.55) & (1.4) & (0.6) \\
 & U & Bias & 0.34 & 0.12 & 0.09 & 0.12 & 0.08 &  & -1.36 & -0.58 & -0.48 & -0.36 & -0.24 \\
 &  & RMSE & (1.38) & (0.38) & (0.28) & (0.27) & (0.22) &  & (2.39) & (0.98) & (0.75) & (0.64) & (0.47) \\
 & Non & Bias & 0.16 & 0.41 & 0.36 & 0.24 & 0.09 &  & -1.31 & -0.74 & -0.69 & -0.61 & -0.22 \\
 &  & RMSE & (2.26) & (1.35) & (1.15) & (0.55) & (0.24) &  & (2.89) & (1.74) & (1.55) & (1.4) & (0.63) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 7.58 & 15.04 & 22.05 & 36.19 & 72.01 & -3.0 & 7.58 & 15.04 & 22.05 & 36.19 & 72.01 \\
 & U,T & Bias & 0.0 & 0.19 & 0.11 & 0.08 & 0.09 &  & -1.7 & -0.94 & -0.62 & -0.43 & -0.37 \\
 &  & RMSE & (2.04) & (0.51) & (0.35) & (0.29) & (0.2) &  & (2.68) & (1.72) & (1.26) & (0.82) & (0.64) \\
 & T & Bias & 0.03 & 0.37 & 0.17 & 0.03 & 0.07 &  & -0.16 & -0.7 & -0.84 & -0.18 & -0.19 \\
 &  & RMSE & (4.37) & (1.78) & (1.43) & (0.26) & (0.17) &  & (4.14) & (2.49) & (2.11) & (0.55) & (0.37) \\
 & U & Bias & -0.01 & 0.17 & 0.09 & 0.06 & 0.08 &  & -1.72 & -0.93 & -0.59 & -0.42 & -0.39 \\
 &  & RMSE & (2.04) & (0.51) & (0.32) & (0.27) & (0.2) &  & (2.68) & (1.71) & (1.22) & (0.82) & (0.63) \\
 & Non & Bias & 0.22 & 0.36 & 0.23 & 0.05 & 0.07 &  & -0.41 & -0.71 & -0.89 & -0.19 & -0.18 \\
 &  & RMSE & (4.46) & (1.78) & (1.55) & (0.28) & (0.19) &  & (4.04) & (2.48) & (2.18) & (0.59) & (0.37) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_with_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.01 & 0.0 & 0.01 & 0.01 \\
 & U,T & Bias & 1.1 & 0.61 & 0.3 & 0.14 & -0.0 \\
 &  & RMSE & (2.63) & (1.81) & (0.81) & (0.52) & (0.33) \\
 & T & Bias & 1.11 & 0.63 & 0.29 & 0.14 & -0.01 \\
 &  & RMSE & (2.63) & (1.82) & (0.81) & (0.52) & (0.33) \\
 & U & Bias & 1.13 & 0.64 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (2.64) & (1.82) & (0.81) & (0.52) & (0.34) \\
 & Non & Bias & 1.13 & 0.64 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (2.64) & (1.82) & (0.81) & (0.52) & (0.34) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.13 & 0.1 & 0.15 & 0.12 & 0.15 \\
 & U,T & Bias & -0.02 & 0.07 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.64) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & T & Bias & -0.02 & 0.07 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.64) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & U & Bias & -0.03 & 0.07 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.64) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & Non & Bias & -0.02 & 0.07 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.64) & (0.46) & (0.18) & (0.12) & (0.07) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 4.1 & 7.79 & 10.83 & 17.53 & 32.65 \\
 & U,T & Bias & -0.46 & -0.51 & -0.27 & -0.11 & 0.0 \\
 &  & RMSE & (1.39) & (1.65) & (1.12) & (0.38) & (0.18) \\
 & T & Bias & -0.29 & -0.12 & -0.04 & -0.04 & -0.01 \\
 &  & RMSE & (0.9) & (0.34) & (0.21) & (0.18) & (0.14) \\
 & U & Bias & -0.46 & -0.47 & -0.28 & -0.11 & -0.0 \\
 &  & RMSE & (1.39) & (1.63) & (1.13) & (0.38) & (0.18) \\
 & Non & Bias & -0.29 & -0.11 & -0.04 & -0.04 & -0.0 \\
 &  & RMSE & (0.9) & (0.32) & (0.21) & (0.18) & (0.1) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.41 & 14.36 & 21.34 & 35.0 & 68.81 \\
 & U,T & Bias & -0.74 & -0.85 & -1.02 & -0.56 & -0.15 \\
 &  & RMSE & (3.74) & (2.59) & (2.41) & (1.69) & (0.84) \\
 & T & Bias & -0.58 & -0.2 & -0.21 & -0.07 & -0.01 \\
 &  & RMSE & (1.25) & (0.6) & (0.53) & (0.28) & (0.25) \\
 & U & Bias & -0.73 & -0.86 & -1.12 & -0.58 & -0.16 \\
 &  & RMSE & (3.74) & (2.59) & (2.51) & (1.71) & (0.86) \\
 & Non & Bias & -0.63 & -0.19 & -0.22 & -0.09 & -0.01 \\
 &  & RMSE & (1.35) & (0.6) & (0.54) & (0.28) & (0.18) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 8.86 & 17.02 & 25.8 & 42.67 & 83.73 \\
 & U,T & Bias & 0.29 & -0.1 & -0.18 & -1.36 & -0.37 \\
 &  & RMSE & (4.67) & (3.84) & (3.84) & (3.16) & (1.59) \\
 & T & Bias & -0.83 & -0.69 & -0.58 & -0.15 & -0.12 \\
 &  & RMSE & (1.92) & (1.76) & (1.4) & (0.55) & (0.45) \\
 & U & Bias & 0.35 & -0.15 & -0.25 & -1.33 & -0.34 \\
 &  & RMSE & (4.67) & (3.86) & (3.87) & (3.18) & (1.61) \\
 & Non & Bias & -0.83 & -0.69 & -0.6 & -0.16 & -0.12 \\
 &  & RMSE & (1.92) & (1.76) & (1.4) & (0.55) & (0.38) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_with_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.01 & 0.0 & 0.01 & 0.01 \\
 & U,T & Bias & 0.21 & 0.45 & 0.09 & 0.02 & 0.01 \\
 &  & RMSE & (1.11) & (1.51) & (0.42) & (0.17) & (0.24) \\
 & T & Bias & 0.23 & 0.46 & 0.11 & 0.02 & 0.02 \\
 &  & RMSE & (1.11) & (1.53) & (0.4) & (0.15) & (0.23) \\
 & U & Bias & 0.35 & 0.46 & 0.09 & 0.02 & 0.01 \\
 &  & RMSE & (1.38) & (1.51) & (0.42) & (0.17) & (0.25) \\
 & Non & Bias & 0.25 & 0.47 & 0.11 & 0.02 & 0.01 \\
 &  & RMSE & (1.13) & (1.53) & (0.4) & (0.15) & (0.24) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.16 & 0.12 & 0.12 & 0.12 & 0.14 \\
 & U,T & Bias & -0.05 & 0.02 & 0.01 & -0.0 & 0.0 \\
 &  & RMSE & (0.33) & (0.19) & (0.1) & (0.06) & (0.05) \\
 & T & Bias & -0.05 & 0.03 & 0.01 & -0.0 & 0.0 \\
 &  & RMSE & (0.33) & (0.19) & (0.1) & (0.06) & (0.04) \\
 & U & Bias & -0.06 & 0.02 & 0.02 & -0.0 & 0.0 \\
 &  & RMSE & (0.33) & (0.19) & (0.11) & (0.07) & (0.04) \\
 & Non & Bias & -0.06 & 0.03 & 0.01 & -0.0 & 0.0 \\
 &  & RMSE & (0.33) & (0.19) & (0.1) & (0.06) & (0.04) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 3.79 & 7.08 & 10.13 & 16.55 & 32.1 \\
 & U,T & Bias & -0.21 & -0.11 & -0.04 & -0.04 & -0.02 \\
 &  & RMSE & (0.46) & (0.32) & (0.21) & (0.18) & (0.16) \\
 & T & Bias & -0.19 & -0.11 & -0.04 & -0.05 & -0.02 \\
 &  & RMSE & (0.49) & (0.38) & (0.17) & (0.17) & (0.11) \\
 & U & Bias & -0.21 & -0.11 & -0.04 & -0.04 & -0.0 \\
 &  & RMSE & (0.46) & (0.32) & (0.21) & (0.18) & (0.1) \\
 & Non & Bias & -0.2 & -0.11 & -0.04 & -0.05 & -0.02 \\
 &  & RMSE & (0.52) & (0.38) & (0.17) & (0.17) & (0.11) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.34 & 14.26 & 21.39 & 35.01 & 68.76 \\
 & U,T & Bias & -0.23 & -0.13 & -0.21 & -0.08 & -0.01 \\
 &  & RMSE & (0.99) & (0.55) & (0.53) & (0.28) & (0.25) \\
 & T & Bias & -0.35 & -0.24 & -0.49 & -0.07 & -0.05 \\
 &  & RMSE & (2.4) & (1.16) & (1.54) & (0.27) & (0.14) \\
 & U & Bias & -0.28 & -0.13 & -0.22 & -0.09 & -0.01 \\
 &  & RMSE & (1.12) & (0.55) & (0.54) & (0.28) & (0.18) \\
 & Non & Bias & -0.36 & -0.25 & -0.48 & -0.09 & -0.06 \\
 &  & RMSE & (2.4) & (1.18) & (1.54) & (0.34) & (0.21) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 8.62 & 16.97 & 25.64 & 42.28 & 83.63 \\
 & U,T & Bias & -1.09 & -0.25 & -0.51 & -0.15 & -0.12 \\
 &  & RMSE & (2.19) & (1.14) & (1.34) & (0.55) & (0.45) \\
 & T & Bias & 0.45 & 0.13 & 0.32 & -0.19 & -0.13 \\
 &  & RMSE & (4.43) & (3.59) & (2.82) & (0.94) & (0.33) \\
 & U & Bias & -1.09 & -0.26 & -0.51 & -0.16 & -0.12 \\
 &  & RMSE & (2.19) & (1.14) & (1.34) & (0.55) & (0.38) \\
 & Non & Bias & 0.45 & 0.1 & 0.28 & -0.17 & -0.1 \\
 &  & RMSE & (4.43) & (3.62) & (2.84) & (0.97) & (0.36) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_without_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.01 & 0.01 \\
 & U,T & Bias & 0.28 & 0.51 & 0.3 & 0.14 & -0.0 \\
 &  & RMSE & (1.36) & (1.64) & (0.81) & (0.52) & (0.33) \\
 & T & Bias & 0.28 & 0.54 & 0.3 & 0.15 & -0.01 \\
 &  & RMSE & (1.35) & (1.66) & (0.81) & (0.52) & (0.33) \\
 & U & Bias & 0.3 & 0.55 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (1.37) & (1.66) & (0.81) & (0.52) & (0.34) \\
 & Non & Bias & 0.31 & 0.55 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (1.37) & (1.66) & (0.81) & (0.52) & (0.34) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.12 & 0.11 & 0.15 & 0.13 & 0.11 \\
 & U,T & Bias & -0.05 & 0.06 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.64) & (0.45) & (0.18) & (0.12) & (0.07) \\
 & T & Bias & -0.05 & 0.06 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.64) & (0.45) & (0.18) & (0.12) & (0.07) \\
 & U & Bias & -0.05 & 0.06 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.64) & (0.45) & (0.18) & (0.12) & (0.07) \\
 & Non & Bias & -0.05 & 0.06 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.64) & (0.45) & (0.18) & (0.12) & (0.07) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 3.9 & 7.29 & 10.77 & 17.7 & 32.8 \\
 & U,T & Bias & -0.77 & -0.51 & -0.27 & -0.1 & 0.01 \\
 &  & RMSE & (2.13) & (1.65) & (1.12) & (0.37) & (0.18) \\
 & T & Bias & -0.29 & -0.12 & -0.04 & -0.04 & -0.01 \\
 &  & RMSE & (0.9) & (0.34) & (0.21) & (0.18) & (0.14) \\
 & U & Bias & -0.8 & -0.5 & -0.28 & -0.11 & -0.0 \\
 &  & RMSE & (2.14) & (1.65) & (1.12) & (0.38) & (0.18) \\
 & Non & Bias & -0.29 & -0.11 & -0.04 & -0.04 & -0.0 \\
 &  & RMSE & (0.9) & (0.32) & (0.21) & (0.18) & (0.1) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.57 & 14.34 & 21.51 & 35.28 & 68.77 \\
 & U,T & Bias & -0.65 & -0.81 & -1.02 & -0.56 & -0.14 \\
 &  & RMSE & (3.69) & (2.49) & (2.41) & (1.69) & (0.84) \\
 & T & Bias & -0.4 & -0.22 & -0.21 & -0.07 & -0.02 \\
 &  & RMSE & (1.16) & (0.61) & (0.53) & (0.28) & (0.25) \\
 & U & Bias & -0.65 & -0.88 & -1.12 & -0.58 & -0.16 \\
 &  & RMSE & (3.69) & (2.59) & (2.51) & (1.71) & (0.86) \\
 & Non & Bias & -0.45 & -0.21 & -0.22 & -0.09 & -0.01 \\
 &  & RMSE & (1.27) & (0.61) & (0.54) & (0.28) & (0.18) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 8.7 & 17.05 & 25.65 & 42.47 & 83.63 \\
 & U,T & Bias & 0.4 & -0.26 & -0.13 & -1.36 & -0.37 \\
 &  & RMSE & (4.63) & (3.77) & (3.83) & (3.16) & (1.59) \\
 & T & Bias & -0.8 & -0.85 & -0.58 & -0.15 & -0.12 \\
 &  & RMSE & (1.91) & (1.93) & (1.4) & (0.55) & (0.45) \\
 & U & Bias & 0.4 & -0.31 & -0.24 & -1.33 & -0.34 \\
 &  & RMSE & (4.63) & (3.79) & (3.87) & (3.18) & (1.61) \\
 & Non & Bias & -0.8 & -0.85 & -0.59 & -0.16 & -0.12 \\
 &  & RMSE & (1.91) & (1.93) & (1.4) & (0.55) & (0.38) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_without_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.02 & 0.0 & 0.01 & 0.01 \\
 & U,T & Bias & 0.92 & 0.61 & 0.3 & 0.15 & -0.0 \\
 &  & RMSE & (2.43) & (1.79) & (0.81) & (0.52) & (0.33) \\
 & T & Bias & 0.92 & 0.63 & 0.3 & 0.15 & -0.01 \\
 &  & RMSE & (2.43) & (1.82) & (0.81) & (0.52) & (0.33) \\
 & U & Bias & 0.95 & 0.64 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (2.43) & (1.82) & (0.81) & (0.52) & (0.34) \\
 & Non & Bias & 0.94 & 0.64 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (2.44) & (1.82) & (0.81) & (0.52) & (0.34) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.16 & 0.12 & 0.16 & 0.11 & 0.13 \\
 & U,T & Bias & -0.03 & 0.08 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (0.37) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & T & Bias & -0.03 & 0.08 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (0.37) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & U & Bias & -0.03 & 0.07 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (0.37) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & Non & Bias & -0.04 & 0.07 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (0.37) & (0.46) & (0.18) & (0.12) & (0.07) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 4.01 & 7.7 & 10.88 & 17.44 & 32.74 \\
 & U,T & Bias & -0.78 & -0.5 & -0.27 & -0.11 & 0.01 \\
 &  & RMSE & (2.15) & (1.64) & (1.12) & (0.38) & (0.18) \\
 & T & Bias & -0.28 & -0.11 & -0.04 & -0.04 & -0.01 \\
 &  & RMSE & (0.88) & (0.32) & (0.21) & (0.18) & (0.14) \\
 & U & Bias & -0.79 & -0.47 & -0.28 & -0.11 & -0.0 \\
 &  & RMSE & (2.14) & (1.63) & (1.12) & (0.38) & (0.18) \\
 & Non & Bias & -0.28 & -0.11 & -0.04 & -0.04 & -0.0 \\
 &  & RMSE & (0.88) & (0.32) & (0.21) & (0.18) & (0.1) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.43 & 14.25 & 21.47 & 35.38 & 68.41 \\
 & U,T & Bias & -0.9 & -0.8 & -0.95 & -0.57 & -0.14 \\
 &  & RMSE & (3.34) & (2.49) & (2.32) & (1.69) & (0.84) \\
 & T & Bias & -0.58 & -0.22 & -0.21 & -0.07 & -0.01 \\
 &  & RMSE & (1.42) & (0.61) & (0.53) & (0.28) & (0.25) \\
 & U & Bias & -0.9 & -0.88 & -1.12 & -0.58 & -0.16 \\
 &  & RMSE & (3.34) & (2.59) & (2.51) & (1.71) & (0.86) \\
 & Non & Bias & -0.64 & -0.21 & -0.22 & -0.09 & -0.01 \\
 &  & RMSE & (1.51) & (0.61) & (0.54) & (0.28) & (0.18) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 8.71 & 17.07 & 25.79 & 42.48 & 83.63 \\
 & U,T & Bias & 0.31 & -0.26 & -0.15 & -1.38 & -0.37 \\
 &  & RMSE & (4.67) & (3.9) & (3.83) & (3.16) & (1.59) \\
 & T & Bias & -0.81 & -0.98 & -0.59 & -0.15 & -0.12 \\
 &  & RMSE & (1.91) & (1.98) & (1.4) & (0.55) & (0.45) \\
 & U & Bias & 0.31 & -0.28 & -0.25 & -1.33 & -0.34 \\
 &  & RMSE & (4.67) & (3.93) & (3.87) & (3.18) & (1.61) \\
 & Non & Bias & -0.81 & -0.98 & -0.6 & -0.16 & -0.12 \\
 &  & RMSE & (1.91) & (1.98) & (1.4) & (0.55) & (0.38) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/ratio_score_results_two_variables_shared_subsidy.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcccccccc}
\toprule 
 & $\beta_1/|\gamma|$ & $\beta_2/|\gamma|$ & $\beta_3/|\gamma|$ & $\beta_4/|\gamma|$ & $\beta_5/|\gamma|$ & $\beta_6/|\gamma|$ & $\beta_7/|\gamma|$ & $\beta_8/|\gamma|$ \\
\midrule 
 &  &  &  &  &  &  &  &  \\
 & 0.046 & 0.28 & 0.123 & -0.438 & -0.021 & 0.242 & -0.018 & 0.16 \\
 &  &  &  &  &  &  &  &  \\
relative level & 2.56 & 15.56 & 6.83 & -24.33 & -1.17 & 13.44 & -1.0 & 8.89 \\
 &  &  &  &  &  &  &  &  \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_HHI_only_shared_subsidy.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcc}
\toprule 
 &  &  \\
 &  & Point Est \\
 &  & [95\% CI] \\
\midrule 
 &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 \\
 &  & (S) \\
HHI$_{b}$ $\times$ HHI$_{t}$ & $\beta_{HHI}$ & -154.12 \\
 &  & [-199.0, -151.0] &  &  &  &  &  &  &  \\
merger cost & -$\gamma$ & -1097.01 \\
 &  & [-1967.4, -24.9] \\
subsidy sensitivity & $\delta$ & 5 \\
 &  &  &  &  &  &  &  &  &  \\
\hline 
$\sharp$ Inequalities (Point) &  & 17870 \\
\% Inequalities &  & 0.899 \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_temp.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcccc}
\toprule 
 &  &  & Value Function &  \\
 &  & Point Estimate & Point Estimate & Point Estimate \\
 &  & [95\% CI Set Identified] & [95\% CI Set Identified] & [95\% CI Set Identified] \\
\midrule 
Measure of economies of scale &  &  &  &  \\
 &  &  &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 & +1 & +1 \\
 &  & (Superconsistent) & (Superconsistent) & (Superconsistent) \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_1$ & 13.84 &  & 68.57 \\
 &  & [61.03, 61.03] &  & [-44.48, -44.48] \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_2$ & 55.23 &  & -31.55 \\
 &  & [81.86, 81.86] &  & [-79.1, -79.1] \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_3$ & 54.32 &  & 89.89 \\
 &  & [88.98, 88.98] &  & [97.95, 97.95] \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_4$ & 96.43 &  & -36.28 \\
 &  & [95.82, 95.82] &  & [-7.64, -7.64] \\
Measure of economies of scope &  &  &  &  \\
 &  &  &  &  \\
share of liner$_{b}$ $\times$ share of liner$_{t}$ & $\beta_5$ &  & -1.12 & -9.23 \\
 &  &  & [-28.83, -28.83] & [-24.74, -24.74] \\
share of tramper$_{b}$ $\times$ share of tramper$_{t}$ & $\beta_6$ &  & -46.63 & -1.3 \\
 &  &  & [-9.61, -9.61] & [-5.93, -5.93] \\
share of special$_{b}$ $\times$ share of special$_{t}$ & $\beta_7$ &  & -67.0 & -76.55 \\
 &  &  & [-23.28, -23.28] & [-14.26, -14.26] \\
share of tanker$_{b}$ $\times$ share of tanker$_{t}$ & $\beta_8$ &  & 5.14 & 4.93 \\
 &  &  & [-32.8, -32.8] & [-15.62, -15.62] \\
 &  &  &  &  \\
 &  &  &  &  \\
merger cost & $\gamma$ & -11.22 & -54.8 & -60.91 \\
 &  & [95.82, 95.82] & [-5.86, -5.86] & [-23.87, -23.87] \\
subsidy sensitivity & $\delta$ & 62.33 & -67.71 & -38.27 \\
 &  & [-17.66, -17.66] & [36.75, 36.75] & [61.86, 61.86] \\
\hline 
$\sharp$ Inequalities in Point Estimate &  & 16464 & 16466 & 16466 \\
\% Inequalities &  & 0.977 & 0.977 & 0.978 \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_temp_200search.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcccc}
\toprule 
 &  &  & Value Function &  \\
 &  & Point Estimate & Point Estimate & Point Estimate \\
 &  & [95\% CI Set Identified] & [95\% CI Set Identified] & [95\% CI Set Identified] \\
\midrule 
Measure of economies of scale &  &  &  &  \\
 &  &  &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 & +1 & +1 \\
 &  & (Superconsistent) & (Superconsistent) & (Superconsistent) \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_1$ & 24.89 &  & 39.81 \\
 &  & [-12.47, 92.92] &  & [-71.07, 96.78] \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_2$ & 87.51 &  & 56.3 \\
 &  & [-88.36, 92.72] &  & [-91.73, 94.87] \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_3$ & 7.54 &  & 92.38 \\
 &  & [-3.09, 99.28] &  & [-71.98, 99.35] \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_4$ & 41.37 &  & -32.99 \\
 &  & [-66.73, 95.98] &  & [-88.97, 89.84] \\
Measure of economies of scope &  &  &  &  \\
 &  &  &  &  \\
share of liner$_{b}$ $\times$ share of liner$_{t}$ & $\beta_5$ &  & -3.16 & -98.35 \\
 &  &  & [-96.43, -4.01] & [-96.8, -1.74] \\
share of tramper$_{b}$ $\times$ share of tramper$_{t}$ & $\beta_6$ &  & -4.76 & -60.45 \\
 &  &  & [-97.02, 0.41] & [-96.21, 2.47] \\
share of special$_{b}$ $\times$ share of special$_{t}$ & $\beta_7$ &  & -95.4 & -65.27 \\
 &  &  & [-93.44, -3.16] & [-98.43, -1.58] \\
share of tanker$_{b}$ $\times$ share of tanker$_{t}$ & $\beta_8$ &  & 3.19 & 2.59 \\
 &  &  & [-99.41, 7.07] & [-98.24, 6.35] \\
 &  &  &  &  \\
 &  &  &  &  \\
merger cost & $\gamma$ & -12.03 & -57.4 & -41.05 \\
 &  & [-66.73, 95.98] & [-95.28, -5.17] & [-89.76, -10.65] \\
subsidy sensitivity & $\delta$ & 64.86 & 48.89 & 10.43 \\
 &  & [-34.71, -7.95] & [-91.21, 96.87] & [-82.22, 88.95] \\
\hline 
$\sharp$ Inequalities in Point Estimate &  & 16461 & 16466 & 16466 \\
\% Inequalities &  & 0.977 & 0.977 & 0.978 \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_temp_robustness.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcccc}
\toprule 
 &  &  & Value Function &  \\
 &  & Point Estimate & Point Estimate & Point Estimate \\
 &  & [95\% CI Set Identified] & [95\% CI Set Identified] & [95\% CI Set Identified] \\
\midrule 
Measure of economies of scale &  &  &  &  \\
 &  &  &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 & +1 & +1 \\
 &  & (Superconsistent) & (Superconsistent) & (Superconsistent) \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_1$ & 40.57 &  & 36.19 \\
 &  & [-15.19, 48.95] &  & [-36.04, 47.85] \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_2$ & 27.4 &  & -33.41 \\
 &  & [-46.77, 48.67] &  & [-48.72, 45.8] \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_3$ & 14.27 &  & 5.49 \\
 &  & [-6.22, 49.75] &  & [-39.01, 49.11] \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_4$ & 48.74 &  & -48.04 \\
 &  & [-26.87, 47.59] &  & [-38.67, 45.8] \\
Measure of economies of scope &  &  &  &  \\
 &  &  &  &  \\
share of liner$_{b}$ $\times$ share of liner$_{t}$ & $\beta_5$ &  & -37.9 & -13.72 \\
 &  &  & [-48.62, -1.95] & [-48.67, -1.14] \\
share of tramper$_{b}$ $\times$ share of tramper$_{t}$ & $\beta_6$ &  & -43.64 & -5.61 \\
 &  &  & [-48.76, 0.33] & [-46.57, 0.69] \\
share of special$_{b}$ $\times$ share of special$_{t}$ & $\beta_7$ &  & -26.8 & -30.12 \\
 &  &  & [-47.92, -1.55] & [-47.23, -1.68] \\
share of tanker$_{b}$ $\times$ share of tanker$_{t}$ & $\beta_8$ &  & 3.51 & 3.6 \\
 &  &  & [-48.82, 3.03] & [-48.45, 2.98] \\
 &  &  &  &  \\
 &  &  &  &  \\
merger cost & $\gamma$ & -13.77 & -38.86 & -38.59 \\
 &  & [-26.87, 47.59] & [-45.89, -4.59] & [-47.29, -6.92] \\
subsidy sensitivity & $\delta$ & 44.66 & 20.39 & -40.16 \\
 &  & [-28.43, -6.13] & [-46.08, 46.17] & [-42.55, 45.76] \\
\hline 
$\sharp$ Inequalities in Point Estimate &  & 16462 & 16466 & 16466 \\
\% Inequalities &  & 0.977 & 0.977 & 0.977 \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_temp_shared_subsidy.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccc}
\toprule 
 &  &  & Value Function &  &  \\
 &  & Point Estimate & Point Estimate & Point Estimate & Point Estimate \\
 &  & [95\% CI Set Identified] & [95\% CI Set Identified] & [95\% CI Set Identified] & [95\% CI Set Identified] \\
\midrule 
Measure of Scale variables &  &  &  &  &  \\
 &  &  &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 & +1 & +1 & +1 \\
 &  & (S) & (S) & (S) & (S) \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_1$ & -31.58 &  & 195.56 &  \\
 &  & [-83.36, 188.76] &  & [-119.16, 180.25] &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_2$ & 72.3 &  & 38.93 &  \\
 &  & [-74.01, 193.06] &  & [-192.35, 191.85] &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_3$ & 105.67 &  & 37.34 &  \\
 &  & [-6.78, 196.47] &  & [-141.96, 194.72] &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_4$ & -94.69 &  & 149.87 & 13.61 \\
 &  & [-170.92, 185.86] &  & [-156.67, 185.45] & [-176.17, 187.8] \\
Measure of Share variables &  &  &  &  &  \\
 &  &  &  &  &  \\
share of liner$_{b}$ $\times$ share of liner$_{t}$ & $\beta_5$ &  & -181.03 & -155.7 & -67.88 \\
 &  &  & [-194.82, 10.56] & [-191.87, 33.84] & [-195.87, 8.22] \\
share of tramper$_{b}$ $\times$ share of tramper$_{t}$ & $\beta_6$ &  & 175.14 & 192.85 & 175.7 \\
 &  &  & [12.1, 197.02] & [-140.73, 197.29] & [-45.53, 197.69] \\
share of special$_{b}$ $\times$ share of special$_{t}$ & $\beta_7$ &  & -24.78 & -27.22 & -4.0 \\
 &  &  & [-196.52, -0.23] & [-194.73, -3.28] & [-190.95, -0.75] \\
share of tanker$_{b}$ $\times$ share of tanker$_{t}$ & $\beta_8$ &  & 164.0 & 80.74 & 74.76 \\
 &  &  & [-188.77, 198.34] & [-188.63, 195.99] & [-168.93, 196.28] \\
 &  &  &  &  &  \\
 &  &  &  &  &  \\
merger cost & -$\gamma$ & -1888.51 & -614.84 & -784.46 & -681.56 \\
 &  & [-1965.04, -376.09] & [-1742.89, -333.77] & [-1830.24, -371.14] & [-1663.55, -371.97] \\
subsidy sensitivity ($s^{\text{shared}}$) & $\delta$ & 5 & 5 & 5 & 5 \\
 &  &  &  &  &  \\
\hline 
$\sharp$ Inequalities in Point Estimate &  & 17870 & 17870 & 17870 & 17870 \\
\% Inequalities &  & 0.905 & 0.906 & 0.906 & 0.906 \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_temp_to_buyer_subsidy.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccc}
\toprule 
 &  &  & Value Function &  &  \\
 &  & Point Estimate & Point Estimate & Point Estimate & Point Estimate \\
 &  & [95\% CI Set Identified] & [95\% CI Set Identified] & [95\% CI Set Identified] & [95\% CI Set Identified] \\
\midrule 
Measure of economies of scale &  &  &  &  &  \\
 &  &  &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 & +1 & +1 & +1 \\
 &  & (S) & (S) & (S) & (S) \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_1$ & 116.27 &  & 195.56 &  \\
 &  & [-82.05, 187.55] &  & [-81.87, 191.56] &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_2$ & -35.09 &  & 38.93 &  \\
 &  & [-78.76, 195.09] &  & [-155.34, 194.35] &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_3$ & 127.81 &  & 37.34 &  \\
 &  & [-4.4, 194.71] &  & [-65.07, 196.93] &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_4$ & 78.85 &  & 149.87 & 119.5 \\
 &  & [-107.76, 192.23] &  & [-134.56, 193.37] & [-103.72, 173.19] \\
Measure of economies of scope &  &  &  &  &  \\
 &  &  &  &  &  \\
share of liner$_{b}$ $\times$ share of liner$_{t}$ & $\beta_5$ &  & -181.03 & -155.7 & -195.73 \\
 &  &  & [-192.97, -19.45] & [-193.6, 20.65] & [-198.34, 5.31] \\
share of tramper$_{b}$ $\times$ share of tramper$_{t}$ & $\beta_6$ &  & 175.14 & 192.85 & 136.91 \\
 &  &  & [24.14, 194.66] & [-112.22, 197.2] & [7.77, 196.46] \\
share of special$_{b}$ $\times$ share of special$_{t}$ & $\beta_7$ &  & -24.78 & -27.22 & -1.41 \\
 &  &  & [-191.57, -2.74] & [-195.53, 2.9] & [-195.65, 1.77] \\
share of tanker$_{b}$ $\times$ share of tanker$_{t}$ & $\beta_8$ &  & 164.0 & 80.74 & 51.27 \\
 &  &  & [-189.45, 194.08] & [-186.65, 191.38] & [-193.85, 190.46] \\
 &  &  &  &  &  \\
 &  &  &  &  &  \\
merger cost & -$\gamma$ & -1893.73 & -614.84 & -784.46 & -419.92 \\
 &  & [-1969.04, -558.98] & [-1907.4, -428.34] & [-1957.19, -502.77] & [-1909.57, -478.2] \\
subsidy sensitivity ($s^{\text{shared}}$) & $\delta$ & 5 & 5 & 5 & 5 \\
 &  &  &  &  &  \\
\hline 
$\sharp$ Inequalities in Point Estimate &  & 17870 & 17870 & 17870 & 17870 \\
\% Inequalities &  & 0.905 & 0.906 & 0.906 & 0.906 \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_two_variables_shared_subsidy.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccccc}
\toprule 
 &  &  &  &  &  &  &  &  &  \\
 &  & Point Est & Point & Point & Point & Point & Point & Point & Point \\
 &  & [95\% CI] & [95\% CI] & [95\% CI] & [95\% CI] & [95\% CI] & [95\% CI] & [95\% CI] & [95\% CI] \\
\midrule 
Scale variables &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 & +1 & +1 & +1 & +1 & +1 & +1 & +1 \\
 &  & (S) & (S) & (S) & (S) & (S) & (S) & (S) & (S) \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_1$ & 48.07 &  &  &  &  &  &  &  \\
 &  & [35.9, 171.8] &  &  &  &  &  &  &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_2$ &  & 19.88 &  &  &  &  &  &  \\
 &  &  & [-30.0, 166.1] &  &  &  &  &  &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_3$ &  &  & 111.48 &  &  &  &  &  \\
 &  &  &  & [42.0, 191.1] &  &  &  &  &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_4$ &  &  &  & -182.85 &  &  &  &  \\
 &  &  &  &  & [-81.0, 198.7] &  &  &  &  \\
Share variables &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_5$ &  &  &  &  & -1.75 &  &  &  \\
 &  &  &  &  &  & [-181.9, -2.2] &  &  &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_6$ &  &  &  &  &  & 18.81 &  &  \\
 &  &  &  &  &  &  & [13.5, 194.4] &  &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_7$ &  &  &  &  &  &  & -6.52 &  \\
 &  &  &  &  &  &  &  & [-182.1, -0.5] &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_8$ &  &  &  &  &  &  &  & 14.75 \\
 &  &  &  &  &  &  &  &  & [12.8, 177.9] \\
 &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  \\
merger cost & -$\gamma$ & -1055.26 & -70.95 & -903.12 & -417.06 & -82.28 & -77.87 & -355.07 & -91.96 \\
 &  & [-1943.3, -491.3] & [-1803.2, -72.8] & [-1941.9, -321.5] & [-1921.1, -90.0] & [-1917.4, -96.8] & [-795.5, -61.5] & [-1867.6, -109.8] & [-791.0, -88.5] \\
subsidy sensitivity & $\delta$ & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 \\
 &  &  &  &  &  &  &  &  &  \\
\hline 
$\sharp$ Inequalities (Point) &  & 17870 & 17870 & 17870 & 17870 & 17870 & 17870 & 17870 & 17870 \\
\% Inequalities &  & 0.9053 & 0.9052 & 0.9053 & 0.9052 & 0.9051 & 0.9059 & 0.905 & 0.9057 \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_two_variables_shared_subsidy_main_firms_only.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccccc}
\toprule 
 &  &  &  &  &  &  &  &  &  \\
 &  & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] \\
\midrule 
Scale variables &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 & +1 & +1 & +1 & +1 & +1 & +1 & +1 \\
 &  & (S) & (S) & (S) & (S) & (S) & (S) & (S) & (S) \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_1$ & [175.7, 175.7] &  &  &  &  &  &  &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_2$ &  & [159.9, 159.9] &  &  &  &  &  &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_3$ &  &  & [-194.1, -194.1] &  &  &  &  &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_4$ &  &  &  & [108.1, 146.2] &  &  &  &  \\
Share variables &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_5$ &  &  &  &  & [149.6, 155.1] &  &  &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_6$ &  &  &  &  &  & [106.1, 199.6] &  &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_7$ &  &  &  &  &  &  & [-199.5, -0.0] &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_8$ &  &  &  &  &  &  &  & [-199.8, -0.0] \\
 &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  \\
merger cost & -$\gamma$ & [-78.9, -78.9] & [-33.3, -33.3] & [-34.5, -34.5] & [-47.2, -40.9] & [-43.6, -41.3] & [-43.4, -28.4] & [-42.2, -17.2] & [-42.3, -17.7] \\
subsidy sensitivity & $\delta$ & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 \\
 &  &  &  &  &  &  &  &  &  \\
\hline 
$\sharp$ Inequalities (Point) &  & 330 & 330 & 330 & 330 & 330 & 330 & 330 & 330 \\
\% Inequalities &  & 0.9055 & 0.8712 & 0.8738 & 0.8807 & 0.8727 & 0.8727 & 0.8576 & 0.8576 \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_two_variables_to_buyer_subsidy_main_firms_only.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccccc}
\toprule 
 &  &  &  &  &  &  &  &  &  \\
 &  & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] \\
\midrule 
Scale variables &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 & +1 & +1 & +1 & +1 & +1 & +1 & +1 \\
 &  & (S) & (S) & (S) & (S) & (S) & (S) & (S) & (S) \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_1$ & [87.9, 87.9] &  &  &  &  &  &  &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_2$ &  & [51.4, 116.0] &  &  &  &  &  &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_3$ &  &  & [-66.2, -66.2] &  &  &  &  &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_4$ &  &  &  & [-192.1, -175.0] &  &  &  &  \\
Share variables &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_5$ &  &  &  &  & [36.9, 36.9] &  &  &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_6$ &  &  &  &  &  & [174.9, 174.9] &  &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_7$ &  &  &  &  &  &  & [155.0, 165.1] &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_8$ &  &  &  &  &  &  &  & [171.0, 171.0] \\
 &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  \\
merger cost & -$\gamma$ & [-12.1, -12.1] & [-14.4, -4.5] & [-5.2, -5.2] & [-4.7, -3.8] & [-15.0, -15.0] & [-7.9, -7.9] & [-7.0, -5.2] & [-10.0, -10.0] \\
subsidy sensitivity & $\delta$ & 500 & 500 & 500 & 500 & 500 & 500 & 500 & 500 \\
 &  &  &  &  &  &  &  &  &  \\
\hline 
$\sharp$ Inequalities (Point) &  & 328 & 328 & 328 & 328 & 328 & 328 & 328 & 328 \\
\% Inequalities &  & 0.9633 & 0.9266 & 0.939 & 0.9146 & 0.9755 & 0.945 & 0.9573 & 0.9512 \\
\bottomrule 
\end{tabular}


==> figuretable/score_results_two_variables_to_buyer_subsidy_main_firms_only_delta_20.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccccc}
\toprule 
 &  &  &  &  &  &  &  &  &  \\
 &  & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] & [LB, UB] \\
\midrule 
Scale variables &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  \\
total$_{b}$ $\times$ total$_{t}$ & $\beta_0$ & +1 & +1 & +1 & +1 & +1 & +1 & +1 & +1 \\
 &  & (S) & (S) & (S) & (S) & (S) & (S) & (S) & (S) \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_1$ & [124.0, 124.0] &  &  &  &  &  &  &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_2$ &  & [54.1, 293.4] &  &  &  &  &  &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_3$ &  &  & [-151.8, -42.6] &  &  &  &  &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_4$ &  &  &  & [-220.8, -220.8] &  &  &  &  \\
Share variables &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  \\
liner$_{b}$ $\times$ liner$_{t}$ & $\beta_5$ &  &  &  &  & [33.9, 37.4] &  &  &  \\
tramper$_{b}$ $\times$ tramper$_{t}$ & $\beta_6$ &  &  &  &  &  & [241.9, 279.9] &  &  \\
special$_{b}$ $\times$ special$_{t}$ & $\beta_7$ &  &  &  &  &  &  & [278.9, 292.6] &  \\
tanker$_{b}$ $\times$ tanker$_{t}$ & $\beta_8$ &  &  &  &  &  &  &  & [286.4, 286.4] \\
 &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  \\
merger cost & -$\gamma$ & [-15.4, -15.4] & [-10.3, -5.2] & [-9.1, -1.8] & [-8.4, -8.4] & [-13.6, -3.5] & [-9.1, -3.8] & [-7.8, -5.2] & [-8.9, -8.9] \\
subsidy sensitivity & $\delta$ & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 \\
 &  &  &  &  &  &  &  &  &  \\
\hline 
$\sharp$ Inequalities (Point) &  & 330 & 330 & 330 & 330 & 330 & 330 & 330 & 330 \\
\% Inequalities &  & 0.9636 & 0.9271 & 0.9394 & 0.9152 & 0.9756 & 0.9514 & 0.9635 & 0.9515 \\
\bottomrule 
\end{tabular}


==> figuretable/tonnage_size_table.tex <==
%latex.default(file = table_name, title = "", booktabs = TRUE,     object = tonnage_table, col.just = rep("r", ncol(tonnage_table)),     center = "none", table.env = FALSE, cgroupTexCmd = "itshape",     colnamesTexCmd = "itshape", collabel.just = rep("r", ncol(tonnage_table)))%
\begin{tabular}{lrrrrrrrr}
\toprule
\multicolumn{1}{l}{\itshape }&\multicolumn{1}{r}{\itshape N}&\multicolumn{1}{r}{\itshape mean}&\multicolumn{1}{r}{\itshape sd}&\multicolumn{1}{r}{\itshape min}&\multicolumn{1}{r}{\itshape q25}&\multicolumn{1}{r}{\itshape q50}&\multicolumn{1}{r}{\itshape q75}&\multicolumn{1}{r}{\itshape max}\tabularnewline
\midrule
1. Liner tonnage (ton)&$127$&20715.795&79300.11&0&0.00&0&0.00&526000\tabularnewline
2. Special tonnage (ton)&$122$&9228.582&19230.33&0&0.00&0&6732.00&98768\tabularnewline
3. Tramper tonnage (ton)&$125$&25452.304&37806.67&0&0.00&9807&27172.00&166102\tabularnewline
4. Tanker tonnage (ton)&$127$&19486.850&43190.61&0&0.00&0&21232.00&250173\tabularnewline
Total tonnage (1+2+3+4)&$120$&76234.758&139752.56&0&7954.25&21816&67694.25&700730\tabularnewline
\bottomrule
\end{tabular}

